Progressive trajectory matching for medical dataset distillation

It is essential but challenging to share medical image datasets due to privacy issues, which prohibit building foundation models and knowledge transfer. In this paper, we propose a novel dataset distillation method to condense the original medical image datasets into a synthetic one that preserves useful information for building an analysis model without accessing the original datasets. Existing methods tackle only natural images by randomly matching parts of the training trajectories of the model parameters trained by the whole real datasets. However, through extensive experiments on medical image datasets, the training process is extremely unstable and achieves inferior distillation results. To solve these barriers, we propose to design a novel progressive trajectory matching strategy to improve the training stability for medical image dataset distillation. Additionally, it is observed that improved stability prevents the synthetic dataset diversity and final performance improvements. Therefore, we propose a dynamic overlap mitigation module that improves the synthetic dataset diversity by dynamically eliminating the overlap across different images and retraining parts of the synthetic images for better convergence. Finally, we propose a new medical image dataset distillation benchmark of various modalities and configurations to promote fair evaluations. It is validated that our proposed method achieves 8.33% improvement over previous state-of-the-art methods on average, and 11.7% improvement when ipc=2 (i.e., image per class is 2). Codes and benchmarks will be released.

==> figures/MMD.tex <==
\begin{figure}[h]
\centering
 \includegraphics[width=2.3in]{Figs/00.pdf}
 \caption{Comparison of the distribution differences of our method to base(w/o overlap) and base(w/ overlap) using the MMD value in the PATHMNIST.}
 \label{01}
\end{figure}

==> figures/fig.tex <==

\begin{figure}[htbp]
        \centering
        \subcaptionbox{mtt}{
        \centering
        \includegraphics[width=3in]{Figs/fig_mtt.png}
    }
        \subcaptionbox{ftd}{
        \includegraphics[width=3in]{Figs/fig_ftd.png}
    }
        \subcaptionbox{overlap}{
        \centering
        \includegraphics[width=3in]{Figs/fig_our_with_overlap.png}
    }
        \subcaptionbox{our}{
        \includegraphics[width=3in]{Figs/fig_our.png}
    }
        \caption{TEST;\chensays{can we link how differences visualized, can help and improve the sub-class accuracies?}}
        \label{fig:11}
\end{figure}
